Hyperspectral Image Super-resolution with Deep Priors and Degradation Model Inversion

To overcome inherent hardware limitations of hyperspectral imaging systems with respect to their spatial resolution, fusion-based hyperspectral image (HSI) super-resolution is attracting increasing attention. This technique aims to fuse a low-resolution (LR) HSI and a conventional high-resolution (HR) RGB image in order to obtain an HR HSI. Recently, deep learning architectures have been used to address the HSI super-resolution problem and have achieved remarkable performance. However, they ignore the degradation model even though this model has a clear physical interpretation and may contribute to improve the performance. We address this problem by proposing a method that, on the one hand, makes use of the linear degradation model in the data-fidelity term of the objective function and, on the other hand, utilizes the output of a convolutional neural network for designing a deep prior regularizer in spectral and spatial gradient domains. Experiments show the performance improvement achieved with this strategy.

==> Hyperspectral image super-resolution with deep priors and degradation model inversion/MathSymbolDefs.tex <==
% mathcal symbol
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cO}{\mathcal{O}}
%\newcommand{\cS}{\mathcal{S}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\cN}{\overline{\mathcal{N}}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}

% boldsymbol capital letters
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}



%boldsymbol small letters
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\boldf}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\boldh}{\boldsymbol{h}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}

%boldsymbol 
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\beps}{\boldsymbol{\epsilon}}
\newcommand{\bSig}{\boldsymbol{\Sigma}}
\newcommand{\bsig}{\boldsymbol{\sigma}}
\newcommand{\bUps}{\boldsymbol{\Upsilon}}
\def\One{\boldsymbol{1}}
\def\Zero{\boldsymbol{0}}

%boldsymbol mathcal
\newcommand{\cA}{\boldsymbol{\cal{A}}}
\newcommand{\cB}{\boldsymbol{\cal{B}}}
\newcommand{\cC}{\boldsymbol{\cal{C}}}
\newcommand{\cD}{\boldsymbol{\cal{D}}}
\newcommand{\cF}{\boldsymbol{\cal{F}}}
\newcommand{\cG}{\boldsymbol{\cal{G}}}
\newcommand{\cH}{\boldsymbol{\cal{H}}}
\newcommand{\cK}{\boldsymbol{\cal{K}}}
\newcommand{\cM}{\boldsymbol{\cal{M}}}
\newcommand{\cP}{\boldsymbol{\cal{P}}}
\newcommand{\cR}{\boldsymbol{\cal{R}}}
\newcommand{\cS}{\boldsymbol{\cal{S}}}
\newcommand{\cQ}{\boldsymbol{\cal{Q}}}
\newcommand{\cT}{\boldsymbol{\cal{T}}}
\newcommand{\cX}{\boldsymbol{\cal{X}}}
\newcommand{\cY}{\boldsymbol{\cal{Y}}}
\newcommand{\cZ}{\boldsymbol{\cal{Z}}}


% boldsymbol with tilde
\newcommand{\bwt}{\widetilde\bw}
\newcommand{\bpsit}{\widetilde\bpsi}
\newcommand{\bphit}{\widetilde\bphi}

% text symbol
\newcommand{\tr}{\text{Tr}}
\newcommand{\vc}{\text{vec}}
\newcommand{\bvc}{\text{bvec}}
\newcommand{\col}{\text{col}}
\newcommand{\sign}{\text{sign}}
\newcommand{\diag}{\text{diag}}
\newcommand{\prox}{\text{prox}}
\newcommand{\proj}{\text{P}}
\newcommand{\card}{\text{card}}
\newcommand{\expec}{\mathbb{E}}


%Operators
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\st}{subject\,to}

\def\R{\ensuremath{{\mathrm{I\!R}}}}
